Active Learning for Semantic Segmentation with Multi-class Label Query

This paper proposes a new active learning method for semantic segmentation. The core of our method lies in a new annotation query design. It samples informative local image regions (e.g., superpixels), and for each of such regions, asks an oracle for a multi-hot vector indicating all classes existing in the region. This multi-class labeling strategy is substantially more efficient than existing ones like segmentation, polygon, and even dominant class labeling in terms of annotation time per click. However, it introduces the class ambiguity issue in training as it assigns partial labels (i.e., a set of candidate classes) to individual pixels. We thus propose a new algorithm for learning semantic segmentation while disambiguating the partial labels in two stages. In the first stage, it trains a segmentation model directly with the partial labels through two new loss functions motivated by partial label learning and multiple instance learning. In the second stage, it disambiguates the partial labels by generating pixel-wise pseudo labels, which are used for supervised learning of the model. Equipped with a new acquisition function dedicated to the multi-class labeling, our method outperforms previous work on Cityscapes and PASCAL VOC 2012 while spending less annotation cost. Our code and results are available at https://github.com/sehyun03/MulActSeg.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sections/_7_rebuttal.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figs/sampling_v2.png}
    \caption{Accuracy in mIoU (\%) versus the number of clicks (budget) for multi-class labeling evaluated on Cityscapes equipped with six different acquisition functions: \sftype{Random}, \sftype{KNN}, \sftype{Margin}, \sftype{BvSB}, \sftype{ClassBal}, and our sampling strategy (\sftype{PixBal}).
    The reported accuracy scores are averaged across three trials.}
\label{fig:sampling}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figs/small_budget_v1.pdf}
    \caption{Accuracy in mIoU (\%) versus the number of clicks (budget) evaluated on Cityscapes using ResNet50 when combined with \sftype{PixBal}.
    We evaluate three budget scenarios: (a) 10K clicks over 5 rounds, (b) 50K clicks over 10 rounds, and (c) 100K clicks over 5 rounds.}
\label{fig:50k_spsize}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figs/sp_size_v1.pdf}
    \caption{Accuracy in mIoU (\%) versus the number of clicks (budget) for multi-class labeling (\sftype{Mul}) and dominant-class labeling (\sftype{Dom}) equipped with \sftype{PixBal} evaluated on Cityscapes using ResNet50.
    (a) Effect of superpixel generation algorithms: \sftype{SEEDS} and \sftype{SLIC}.
    (b) Effect of superpixel sizes: 16$\times$16 (\sftype{sp16}), 32$\times$32 (\sftype{sp32}), and 64$\times$64 (\sftype{sp64}).}
\label{fig:spx_quality}
\end{figure}
